Acceleration of cosmic rays in presence of magnetohydrodynamic fluctuations at small scales

This work investigates the evolution of the distribution of charged particles due to the mechanism of stochastic turbulent acceleration (STA) in presence of small-scale turbulence with a mean magnetic field. STA is usually modelled as a biased random walk process in the momentum space of the non-thermal particles. This results in an advection-diffusion type transport equation for the non-thermal particle distribution function. Under quasilinear approximation, and by assuming turbulent spectra with power being available only in the sub-gyroscale range, we find that the Fokker-Planck diffusion coefficients $D_{\gamma\gamma}$ and $D_{\mu\mu}$ scale with the Lorentz factor $\gamma$ as: $D_{\gamma\gamma}\propto\gamma^{-2/3}$ and $D_{\mu\mu}\propto\gamma^{-8/3}$. We consider Alfv\`{e}n and fast waves in our calculations, and find a universal trend for the momentum diffusion coefficient irrespective of the properties of the small-scale turbulence. Such universality has already been reported regarding the spatial diffusion of the cosmic rays, and, here too, we observe a universality in the momentum diffusion coefficient. Furthermore, with the calculated transport coefficients, we numerically solve the advection-diffusion type transport equation for the non-thermal particles. We demonstrate the interplay of various mircophysical processes such as STA, synchrotron loss and particle escape on the particle distribution by systematically varying the parameters of the problem. We observe that the effect of the small-scale turbulence is more impactful for the high energy protons as compared to the electrons and such turbulence is capable of sustaining the energy of the protons from catastrophic radiative loss processes. Such a finding is novel and helps us to enhance our understanding about the hadronic emission processes that are typically considered as a competitor for the leptonic emission.

==> calculations.tex <==
\section{Calculation of the transport coefficients due to small-scale turbulence} \label{sec:calc} 

In this section, we provide the derivation of the momentum transport coefficients $D_{pp}$, $D_{\mu\mu}$ and $D_{\mu p}$ due to sub-gyroscale perturbations in the presence of a mean magnetic field, where $p$ and $\mu$ are the momentum and pitch-angle of the non-thermal particles, respectively.
We begin with the following form of the diffusive transport coefficients in momentum space \citep{schlickeiser_1993}:
\begin{eqnarray}
\left[ \begin{array}{c}
D_{\mu\mu}\\
D_{\mu p}\\
D_{pp}
\end{array}\right] = {\Omega ^{2}(1-\mu ^{2})\over 2B_{0}^{2}}\left[ \begin{array}{c}
1\\
mc\\
m^{2}c^{2}
\end{array}\right] {\mathcal{R}}e \sum _{n=-\infty }^{n=\infty }
\int_{k_{\rm min}}^{k_{\rm max}}\, d^{3}\vec{k}
\int _{0}^{\infty }dte^{-\iota(k_{\parallel }v_{\parallel }-\omega +n\Omega )t} \left\{ J_{n+1}^{2}\left({k_{\perp }v_{\perp }\over \Omega }\right)\left[ \begin{array}{c}
P_{{\cal RR}}({\vec{k}})\\
T_{{\cal RR}}({\vec{k}})\\
R_{{\cal RR}}({\vec{k}})
\end{array}\right] \right. \nonumber \\
+ J_{n-1}^{2}\left({k_{\perp }v_{\perp }\over \Omega }\right) \left[ \begin{array}{c}
P_{{\cal LL}}({\vec{k}})\\
-T_{{\cal LL}}({\vec{k}})\\
R_{{\cal LL}}({\vec{k}})
\end{array} \right] + J_{n+1}\left({k_{\perp }v_{\perp }\over \Omega }\right)J_{n-1}\left({k_{\perp }v_{\perp }\over \Omega }\right)
\left. \left[ e^{\iota 2\phi }\left[ \begin{array}{c}
-P_{{\cal RL}}({\vec{k}})\\
T_{{\cal RL}}({\vec{k}})\\
R_{{\cal RL}}({\vec{k}})
\end{array}\right] +e^{-\iota 2\phi }\left[ \begin{array}{c}
-P_{{\cal LR}}({\vec{k}})\\
-T_{{\cal LR}}({\vec{k}})\\
R_{{\cal LR}}({\vec{k}})
\end{array}\right] \right] \right\} \label{eq:QLTdiff} 
\end{eqnarray}
%
%NS: made it ; separated
where $\Omega = \Omega_{NR}/\gamma$ and $m=\gamma m_e$ are the gyro-frequency and mass of the relativistic non-thermal particle (electron for our case), respectively;
$\Omega_{NR}$ denotes the non-relativistic gyro-frequency and
$\gamma$ is the Lorentz factor;
wave number $k_{\rm min}$ corresponds to the inverse of some maximal length scale L as $k_{\rm min}=2\pi L^{-1}$,
and $k_{\rm max}$ corresponds to the dissipation scale\ns{;} $v_{\perp }$ {and $k_{\perp}$ are} the particle's velocity and the wave vector components perpendicular to the mean magnetic field $\bfB_0 = B_0 \hat{z}$;
$\phi$ represents the phase angle between the Cartesian components of the wave vector
in a plane perpendicular to the mean magnetic field, i.e., $\phi =\tan^{-1} (k_{y}/k_{x})$;
${\cal L}$ and ${\cal R}$ represent left and right hand polarizations,
given by ${\cal L},{\cal R}=(x\pm \iota y)/\sqrt{2}$, with $x$ and $y$ being the Cartesian coordinates, and $\iota=\sqrt{-1}$ is the imaginary number;
$J_{n}(:)$ is the Bessel function of first kind with integer order $n$. 
% and ${\cal L},{\cal R}=(x\pm \iota y)/\sqrt{2}$ represent left and right hand polarization.
Note that the {diffusive transport} coefficients in Eq.~(\ref{eq:QLTdiff}) corresponds to the lowest order in $V_{A}/c$ with $V_{A}$ being the Alfv\'en velocity. The above transport coefficients are only valid for Alfv\'en modes, whereas for other compressible modes, additional terms are needed to be considered in the equation for $D_{\mu p}$.
Here we focus only on Alfv\'{e}n waves because of their damping free nature in fully ionised medium \citep{kulsrud_1969,Ginzburg_1970,yan_2002}.
Further, the terms $P_{{ij}}$, $T_{{ij}}$, $Q_{ij}$ and $R_{{ij}}$ are defined using two point correlations at scales $\vec{k}$ and $\vec{k'}$ as follows, 
\begin{eqnarray} \label{eq:corr}
\left\langle B_i(\vec{k})B_j^{*}(\vec{k'})\right\rangle=\delta (\vec{k}-\vec{k'})P_{ij }(\vec{k}), \nonumber \\
\left\langle B_i(\vec{k})E_j^{*}(\vec{k'})\right\rangle=\delta (\vec{k}-\vec{k'})T_{ij }(\vec{k}), \nonumber \\
\left\langle E_i(\vec{k})B_j^{*}(\vec{k'})\right\rangle=\delta (\vec{k}-\vec{k'})Q_{ij }(\vec{k}), \nonumber \\
\left\langle E_i(\vec{k})E_j^{*}(\vec{k'})\right\rangle=\delta (\vec{k}-\vec{k'})R_{ij }(\vec{k}).
\end{eqnarray}
where $B_{i}$ {and $E_{i}$ are} the magnetic {and electric} field fluctuations.
%
We also define terms $C_{{ij}}$ and $Y_{ij}$ that relate the magnetic field and velocity correlations as follows:
\begin{eqnarray}\label{eq:red_corr}
%\left\langle B_i(\vec{k})B_j^{*}(\vec{k'})\right\rangle/B_{0}^{2}=\delta (\vec{k}-\vec{k'})M_{ij }(\vec{k}), \nonumber \\
\left\langle u_i(\vec{k})B_j^{*}(\vec{k'})\right\rangle/V_{A}B_{0}=\delta (\vec{k}-\vec{k'})C_{ij }(\vec{k}), \nonumber \\
\left\langle u_i(\vec{k})u_j^{*}(\vec{k'})\right\rangle/V_{A}^{2}=\delta (\vec{k}-\vec{k'})Y_{ij }(\vec{k}),
\end{eqnarray}

Further considering MHD turbulence, the Ohm's Law implies $\mathbf{E}(\vec{k})=-\frac{\mathbf{u}(\vec{k})}{c}\times \mathbf{B}_{0}$ {with $\mathbf{u}(\vec{k})$ being the Fourier component of the velocity fluctuation of the underlying MHD flow.} 
Adopting this expression of electric field in Eq~(\ref{eq:corr}) and using the definitions provided in Eq.~(\ref{eq:red_corr})
we obtain, 
\begin{eqnarray}\label{eq:corr_mhd}
T_{ij }(\vec{k})=-\frac{B_{0}^{2}V_{A}}{c}\epsilon_{jpz}C_{ip}\left(\vec{k}\right), \nonumber \\
Q_{ij }(\vec{k})=-\frac{B_{0}^{2}V_{A}}{c} \epsilon_{imz}C_{mj}\left(\vec{k}\right), \nonumber \\
R_{ij }(\vec{k})=\frac{B_{0}^{2}V_{A}^{2}}{c^2}\left[\delta_{ij}Y_{pp}\left(\vec{k}\right)-Y_{ji}\left(\vec{k}\right)\right]
\end{eqnarray}
%
{where, $z$ is the Cartesian coordinate along the mean magnetic field (see appendix~\ref{sec:appendix1} for detailed derivation). }


For the small-scale turbulence we consider a single scale Dirac $\delta$ turbulent energy injection of the following form,
\begin{eqnarray}\label{eq:turb_spec}
    Y_{ij}\left(\vec{k}\right) = \left(\delta_{ij}-\frac{k_{i}k_{j}}{k^2}\right)P_{0}\delta\left(\frac{k}{m'k_{g}}-1\right)\,k^{-2}
\end{eqnarray}
where, $k_{g}$ is the inverse of the non-relativistic gyro-radius of a charged particle, $k_{g}=\Omega_{NR}/v_{\perp}$, and $m'$ is a parameter which dictates the scale of the turbulent energy injection. 
The motivation behind using such kind of turbulence spectra can be attributed to the fact that owing to the high rigidity, the cosmic ray particles will be very weakly dependent on the form of the turbulence spectrum \citep[][]{subedi_2017}.
Therefore any other form of $Y_{ij}$ is expected not to alter the result very much. 
An estimation of $P_{0}$ in the definition of turbulent spectrum can be computed following the equipartion of magnetic energy,
\begin{eqnarray}\label{eq:equipartition}
    \int d^{3}\vec{k} Y_{ii}\frac{\rho V_{A}^{2}}{2}\sim \frac{B_{0}^{2}}{8\pi}
\end{eqnarray}
with $\rho$ being the density and $V_{A}=B_{0}^{2}/(4\pi\rho)$ is the Alfv\'{e}n velocity.
Comparing the value of the integration on the left side to the right side results in $P_{0}\sim(8\pi m'k_{g})^{-1}$.
On substituting the correlation coefficients for MHD turbulence (Eqs.~\ref{eq:corr} and \ref{eq:corr_mhd}) in Eq.~(\ref{eq:QLTdiff}), we obtain the expression of $D_{pp}$ as follows (see appendix~\ref{sec:appendix2})
\begin{eqnarray}\label{eq:Dppinitial}
\nonumber
    D_{pp} = \frac{\Omega^2\left(1-\mu^2\right)}{2B_{0}^2}m^2c^2\frac{B_{0}^{2} V_{A}^{2}}{c^{2}}P_{0}\mathcal{R}e\left[\sum_{n = -\infty}^{\infty}\int_{k_{min}}^{k_{max}}\delta\left(\frac{k}{m'k_{g}}-1\right)k^{-2}d^{3}\vec{k} \int_{0}^{\infty}dt\,\,e^{-\iota\left(k_{||}v_{||}-\omega+n\Omega\right)t}
    \left\{J_{n+1}^2\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)\left(1+\frac{k_{\perp}^{2}}{2k^{2}}\right)\right .\right .\\
    \left .\left .\nonumber +J_{n-1}^2\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)\left(1+\frac{k_{\perp}^{2}}{2k^{2}}\right)+ 
    J_{n+1}\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)J_{n-1}\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)\left( e^{2\iota\psi}\frac{1}{2} \frac{k_{\perp}^{2}}{k^{2}} e^{-2\iota\psi} +e^{-2\iota\psi}\frac{1}{2} \frac{k_{\perp}^{2}}{k^{2}} e^{2\iota\psi}\right) \right\}\right] \\
    \nonumber
    = \frac{\Omega^2\left(1-\mu^2\right)}{2}m^2c^2\frac{V_{A}^{2}}{c^{2}}P_{0}\mathcal{R}e\left[\sum_{n = -\infty}^{\infty}\int_{k_{min}}^{k_{max}}\delta\left(\frac{k}{m'k_{g}}-1\right)k^{-2}d^{3}\vec{k} \int_{0}^{\infty}dt\,\,e^{-\iota\left(k_{||}v_{||}-\omega+n\Omega\right)t}
    \left\{\left(J_{n+1}^2\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)+J_{n-1}^2\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)\right)\left(1+\frac{k_{\perp}^{2}}{2k^{2}}\right) \right .\right.
    \\ \left .\left. 
    +J_{n+1}\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)J_{n-1}\left(\frac{k_{\perp}v_{\perp}}{\Omega}\right)\frac{k_{\perp}^{2}}{k^{2}} \right\}\right]
\end{eqnarray}
%
%
%
On performing the integration, $D_{pp}$ simplifies to (see appendix~\ref{sec:appendix3}),
\begin{eqnarray}\label{eq:Dppfinal}
\nonumber
    D_{pp} \simeq \Omega\left(1-\mu^2\right)m^2c^2\frac{V_{A}^{2}}{c^{2}}\pi^{2}{m'}k_{g} P_{0}\mathcal{R}e\left[ \int_{-1}^{1}dx
    \left\{\left(J_{\frac{\omega}{\Omega}-\frac{m'k_{g}xv\mu}{\Omega}+1}^2\left(\frac{m'k_{g}v}{\Omega}\sqrt{1-x^2}\sqrt{1-\mu^2}\right)\right.\right.\right. \\ \nonumber
    \left.\left.\left.
    +J_{\frac{\omega}{\Omega}-\frac{m'k_{g}xv\mu}{\Omega}-1}^2\left(\frac{m'k_{g}v}{\Omega}\sqrt{1-x^2}\sqrt{1-\mu^2}\right)\right)\left(\frac{3-x^{2}}{2}\right) \right.\right. \\ \left.\left.
    +\left(1-x^{2}\right)J_{\frac{\omega}{\Omega}-\frac{m'k_{g}xv\mu}{\Omega}+1}\left(\frac{m'k_{g}v}{\Omega}\sqrt{1-x^2}\sqrt{1-\mu^2}\right)J_{\frac{\omega}{\Omega}-\frac{m'k_{g}xv\mu}{\Omega}-1}\left(\frac{m'k_{g}v}{\Omega}\sqrt{1-x^2}\sqrt{1-\mu^2}\right) \right\}\right].
\end{eqnarray}
%
The above expression for $D_{pp}$ consists of several integrations involving Bessel function within the limits of $\pm 1$ and analytical solutions of such integrations are very challenging. 
We, therefore, consider integrating the above expression numerically to obtain the functional form of $D_{pp}$. 
For that we further simplify Eq.(\ref{eq:Dppfinal}) by noting that the major contribution from the Bessel functions would come when,
$$\frac{\omega}{\Omega}-\frac{m'k_{g}xv\mu}{\Omega}\pm 1 \simeq \frac{m'k_{g}v}{\Omega}\sqrt{1-x^2}\sqrt{1-\mu^2} \gg 1 $$ 
which implies an analogous resonance condition of the following form: $$\omega-m'\vec{k}_{g}\vec{v} \simeq \mp \Omega.$$
Furthermore, note that the presence of $\simeq$ in the above equation indicates {that this condition has to be weakly satisfied.
Therefore, we introduce a parameter in order to modulate the value of $(\omega-m'\vec{k}_{g}\vec{v} \pm \Omega)$ i.e., to broaden the resonance condition.} 
The presence of this resonance condition constrains the limit of the $x$ integral in Eq.~(\ref{eq:Dppfinal}). 
To identify the limits for Alfv\'{e}n waves, we undertake the following exercise: The resonance condition due to the shear Alfv\'{e}n wave, $(\omega = k_{||}V_{A} = kxV_{A})$, becomes,
%
\begin{eqnarray}
\label{eq:constraint}
\nonumber
\frac{\gamma m' k_{g} V_{A} x}{\Omega_{NR}} - \frac{m' k_{g} c \sqrt{1-\frac{1}{\gamma^2}}\mu x}{\Omega_{NR}}\gamma - \frac{m' k_{g}c \sqrt{1-\frac{1}{\gamma^2}}}{\Omega_{NR}}\gamma \sqrt{1-x^2}\sqrt{1-\mu^2} \simeq \mp 1 \\ 
\implies Ax-Bx-G\sqrt{1-x^2} = Q,
\end{eqnarray}
%
where the form of $A$, $B$ and $G$ are as follows,
$$A = \frac{\gamma m' \Omega_{NR} V_{A}}{\Omega_{NR}v_{\perp}} = \frac{\gamma \beta_{A} m'}{\sqrt{1-\frac{1}{\gamma^2}}\sqrt{1-\mu^2}};\quad B = \frac{m' \Omega_{NR} c\gamma \mu}{\Omega_{NR}v_{\perp}} \sqrt{1-\frac{1}{\gamma^2}} = \frac{\gamma \mu m'}{\sqrt{1-\mu^2}};\quad G = \frac{m' \Omega_{NR} c\gamma}{\Omega_{NR}v_{\perp}} \sqrt{1-\frac{1}{\gamma^2}} \sqrt{1-\mu^2} = m' \gamma, $$
with $\beta_{A}$ being the Alfv\'{e}n velocity normalized to $c$, $\beta_{A}=V_{A}/c$.
Note that we have used the definition of $k_{g}$, while defining $A$, $B$ and $G$.
Further with the presence of $Q$, the resonance broadening effect can also be considered.
Eq.~(\ref{eq:constraint}) is a quadratic equation which has solutions of the following form,
\begin{eqnarray}\label{eq:solutionx}
    x[Q] = \frac{\sqrt{A^2G^2 - 2ABG^2 + B^2G^2 + G^4 - G^2Q^2} + AQ - BQ}{A^2 - 2AB + B^2 + G^2};\quad\Tilde{x}[Q] = - x[Q].
\end{eqnarray}
Following the solution of $x$ from Eq.~(\ref{eq:solutionx}), we write the form for $D_{pp}$ in the following way, 
% Following such an exercise, we can write the form for $D_{pp}$ as,
\begin{eqnarray}\label{eq:dpp}
\nonumber
    \frac{D_{pp}}{m_{e}^2c^2}=D_{\gamma\gamma} \simeq \Omega_{NR}^{2}\left(1-\mu^2\right)\gamma\beta_{A}^2\pi^{2}\frac{m'}{c} P_{0}\mathcal{R}e\left[ \int_{\min\{\mathcal{F}\}}^{\max\{\mathcal{F}\}}dy\,
    \left\{\left(J_{(A-B)y+1}^2\left(G\sqrt{1-y^2}\right)
    +J_{(A-B)y-1}^2\left(G\sqrt{1-y^2}\right)\right)\left(\frac{3-y^{2}}{2}\right) \right.\right. \\ \left.\left.
    +\left(1-y^{2}\right)J_{(A-B)y+1}\left(G\sqrt{1-y^2}\right)J_{(A-B)y-1}\left(G\sqrt{1-y^2}\right) \right\}\right].
\end{eqnarray}
%
where $\mathcal{F}=\{x[-1-\sigma],x[-1+\sigma],x[1-\sigma],x[1+\sigma]\}$, with $\sigma$ being the broadening {parameter}.
% The limit of the integration could also be chosen from the other solution, $\Tilde{x}$, which would consider the velocity of Alfv\`en waves from 
% The limit is arbitrary as one could have chosen the other solution for $x=\Tilde{x}$ and could have computed the limits.
% However, the solution won't be affected in such a case as it would consider the direction of propagation of the Alfv\`en wave opposite from what we consider in this work. 
% As it is obvious from Eq.~(\ref{eq:constraint}), $x$ has a parabolic (second order) dependency on $Q$, so this process could lead to $D_{\rm pp}<0$.
% To resolve this discrepancy we discretize $Q\in\{Q-\sigma,Q+\sigma\}$ and compute the value for $x$ from Eq.~(\ref{eq:solutionx}) and compute the Bessel functions. 
% Therefore to avoid this we further sort the computed $x$ values from $Q$ and evaluate the integrals. 
% Solving of Eq.~(\ref{eq:dpp}) analytically is hard because of the presence of the bessel functions, therefore we consider numerical integration to investigate the functional form for $D_{pp}$ for a set of values for $\kappa,\, \beta_{A}\, \text{and}\, \sigma$.
{We solve Eq.~(\ref{eq:dpp}) for different values of $m',\, \beta_{A}\, \text{and}\, \sigma$ and the} result of the numerical integration is discussed in section~\ref{sec:dpp}.

Now we proceed to compute the form of $D_{\mu\mu}$
considering the correlation tensor $P_{ij}=B_{0}^{2}Y_{ij}$.
Such an assumption for the correlation function is typically used for Alfv\'{e}n waves \citep[see for example][]{yan_2002}.
With this correlation function and an exactly similar kind of calculation as shown in appendix~\ref{sec:appendix2} $\&$ \ref{sec:appendix3} leads to the following form for $D_{\mu\mu}$,
\begin{eqnarray}\label{eq:dmumu}
\nonumber
    D_{\mu\mu} \simeq \Omega_{NR}^{2}\left(1-\mu^2\right)\pi^{2}\frac{m'}{\gamma c} P_{0}\mathcal{R}e\left[ \int_{\min\{\mathcal{F}\}}^{\max\{\mathcal{F}\}}dy\,
    \left\{\left(J_{(A-B)y+1}^2\left(G\sqrt{1-y^2}\right)
    +J_{(A-B)y-1}^2\left(G\sqrt{1-y^2}\right)\right)\left(\frac{1+y^{2}}{2}\right) \right.\right. \\ \left.\left.
    +\left(1-y^{2}\right)J_{(A-B)y+1}\left(G\sqrt{1-y^2}\right)J_{(A-B)y-1}\left(G\sqrt{1-y^2}\right) \right\}\right].
\end{eqnarray}
%
Here also, due to the presence of the Bessel function, we consider numerical integration. 
Interestingly, owing to the isotropic nature of the turbulence, all the components of the correlation function for $D_{\mu p}$ come out to be imaginary (see appendix~\ref{sec:appendix2}).
Therefore, $D_{\mu \gamma}=D_{\mu p}/(m_{e}c)$ does not make any contribution toward the transport of these non-thermal particles.
% Interestingly all the correlation function for $D_{\mu p}$ come out to be imaginary (see appendix~\ref{sec:appendix2}) implying $D_{\mu p}=0$. 


==> discussion.tex <==
\section{Summary and discussion}\label{sec:diss}
In this work we consider the effect of small-scale turbulence with a guided magnetic field on the acceleration of very high-energy charged particles.
This study is motivated primarily by an academic interest where our
emphasis is towards understanding the nature of interaction between
the cosmic rays and the stochastic magnetic fields at scales smaller than the particles'
gyro-radius corresponding to the uniform guided magnetic field.
It is likely that such kind of situations occur in various astrophysical scenarios,
for example in the vicinity of relativistic shocks, or when a very high-energy cosmic ray
with gyro-radius larger than the scale of our galaxy passes through.
We carry out a semi-analytic study based on the quasilinear theory of plasma and
determine the momentum transport coefficients due to an isotropic and monochromatic
injection of stochastic magnetic fields at small scales.
Our calculation indicates that in such a situation the transport coefficients follow an inverse power-law trend with the energy, or in other words, the Lorentz factor $\gamma$, of the
charged particles.
In the present work, we obtain the following power law scaling relations for
the turbulent transport coefficients: $D_{\gamma\gamma}\propto\gamma^{-2/3}$,
$D_{\mu\mu}\propto\gamma^{-8/3}$, and $D_{\mu\gamma}=0$.
The earlier work by \cite{tsytovich_1977} reports a power law behaviour of $D_{\gamma \gamma}\propto \gamma^{-1}$ which is different from what we observe here.
The calculated form for $D_{\mu \mu}$ leads to a parallel spatial diffusion coefficient which scales with $\gamma$ as $\sim\gamma^{8/3}$; see Eq.~(\ref{eq:kas}) for $\mathcal{K}$.
Such a parallel diffusion is similar to that of obtained from numerical simulation by \cite{cesse_2001}.
Their result shows that the parallel diffusion in quasilinear regime scales with rigidity (or $\gamma$) with an exponent of $7/3$ which is close to the result that we obtain from asymptotic expansion of the quasilinear diffusion coefficients.
% by considering the magnetostatic slab turbulence spectrum for the magnetic field correlation \citep[see Eq.~2.13 and 4.33 of][]{shalchi_2020}.
% It should be noted that the isotropic monochromatic turbulence injection spectrum considered in the current work is fundamentally different from the anisotropic slab turbulence spectrum, which might be the reason behind the difference between the parallel diffusion coefficients.}

Having obtained these transport coefficients, we then solve the transport equation
for the cosmic rays, i.e., the Fokker-Planck equation.
When we ignore the synchrotron loss and diffusive escape mechanisms,
we find that the small-scale turbulence leads to the energization of
particles in such a way that the low energy particles are accelarated
faster compared to the particles with higher $\gamma$, resulting thus in a
non-uniform acceleration of the cosmic ray particles.
A qualitative comparison with the case where the gyro-radius of particle is smaller than the turbulence correlation length reveals that the acceleration due to small-scale turbulence is relatively less efficient.

We further demonstrate the interplay of various micro-physical processes, such as acceleration, synchrotron loss and diffusive particle escape, on the particle spectrum in various
regimes of the parameters $a$ and $b$ in Eq.~(\ref{eq:transport}).
The particle spectrum is observed to attain a steady-state as a result of the competition between acceleration and synchrotron loss. 
Additionally, with the particle escape process included, the distribution function
evolves in such a way that the high-energy particles leak out of the system faster than the low-energy ones.

Our study indicates that in a situation where small-scale turbulence is mediated by a mean magnetic field, acceleration of high energy particles would be small
in presence of other more dominant competing micro-physical processes, such as
the synchrotron loss and diffusive escape.
However, such an acceleration is found to be significant for lower energy particles.
The hump like structure that develops in the distribution
function signifies the acceleration of low-$\gamma$ particles.
We envisage that in some cases with appropriate values for the dynamical quantities this acceleration could become significant and it may help the non-thermal particles to sustain their energy against the radiative cooling mechanisms.
% \sk{The interplay of various micro-physical processes shown in this academic demonstration could contribute in building a sub-grid model for trnasport of very high energy cosmic rays}

This work is only a first step towards studying a more complex interplay of various micro-physical processes and their impact on the energy spectrum of the cosmic ray.
Other acceleration scenarios where resonant interaction between turbulent waves and high energy cosmic ray particles is not included, for example, adiabatic acceleration due to random velocity of the MHD fluid \citep{ptuskin_1988,lemoine_2019} could also provide significant acceleration to the non-thermal particles with high rigidity.
Such acceleration configurations along with various energy loss processes will be considered in future works. 
As an extension to this present work, it would be interesting to see the effects of small-scale turbulence on the high energy non-thermal particles in a non-linear framework of wave-particle interaction \citep{beresnyak_2011,yan_2008}.
This will be taken up as a future work along with the resonant acceleration due to magnetosonic waves \citep{chandran_2003}.

\section*{DATA AVAILABILITY}
The codes used in this work are available from the corresponding author
upon reasonable request.


==> intro.tex <==
\section{Introduction}
%
The transport of non-thermal charged particles dictates the emission properties of various highly energetic astrophysical sources. 
Usually, this transport phenomenon is mediated by a turbulent magnetic field, which subsequently leads the particles to exhibit diffusive behaviour in both space and energy domains. 
Such a diffusive behaviour in energy is a crucial component in accelerating the particles via the Fermi mechanism since the efficiency and the rate of particle acceleration directly depend on the scattering due to the random magnetic fields.
This turbulent acceleration is speculated to occur in different astrophysical sources with a diverse set of physical conditions, from the solar atmosphere \citep{petrosian_2004,selkowitz_2004,bian_2012} up to more exotic objects, e.g. blazars, gamma-ray bursts and other relativistic outflows \citep{bykov_1996,tramacere_2011,lemoine_2016,asano_2016,xu_2017,asano_2018,xu_2019}.
The magnetic turbulence also dictates the confinement of these charged particles in various astrophysical systems \citep{vukcevic_2007,shalchi_2009}

An analytical quasilinear model of diffusion \citep{jokipii_1966,jokipii_1973} has often been used to estimate diffusion coefficients when the turbulent field is weaker than the background magnetic field.
Such analytical approach has been invoked to study the acceleration of particles via various MHD modes [by Alfv\'{e}n modes \citep{schlickeiser_1989,chandran_2000,cho_2006}; by compressive modes \citep{schlickeiser_1998,yan_2002,chandran_2003}].
% \sk{The quasilinear theory is a first order perturbation theory and it is known to give rise to theoretical problems in diffusion of charged particles in the perpendicular direction to the guided field. }
For strong turbulence, on the other hand, several studies have employed numerical simulations to examine the transport properties of charged particles \citep{giacalone_1999,cesse_2001,candia_2004,fatuzzo_2010}. 
Most of these researchers have focused their attention on the situation in which large-scale turbulence cascades toward smaller dissipative scales and the interaction between turbulent waves and charged particles is mediated by particular resonance conditions. 
Further, in such studies, it is also implicitly assumed that the particles’ gyro-radius is smaller than the maximum scale of the turbulence spectrum. 

However, under several astrophysical circumstances, the particle’s gyro-radius can surpass the maximum coherence length of the turbulence. 
For instance, the transport of supra-thermal particles in the vicinity of a relativistic shock, the propagation of very high-energy cosmic rays within a galaxy, the transport of particles through a medium of active magnetic reconnection, where the generation of small-scale turbulence is governed by the dissipation of magnetic energy, etc. 
Despite the wide application of this regime in several astrophysical systems, it has gained little attention to date. 
Although some recent research has been devoted to studying this under-explored field, it has primarily focused on the problem of spatial transport \citep{cesse_2001}. 
For example, \cite{plotnikov_2011} developed an analytical formulation of the spatial transport coefficients compatible with the numerical results for an intense small-scale random magnetic field. 
Furthermore, the work by \cite{subedi_2017} is worth noting, which studies charged particle diffusion in three-dimensional isotropic turbulent magnetic fields without a mean field.




% Transport of non-thermal charged particles are known to dictate the emission properties of various highly energetic astrophysical sources. 
% Usually this transport phenomena is mediated by a turbulent magnetic field, which subsequently leads the particles to exhibit diffusive behaviour in both space and energy domains.
% Such a diffusive behaviour in energy is a crucial component in accelerating the particles via Fermi mechanism, since the efficiency and the rate of particle acceleration directly depend on the scattering due to the random magnetic fields.
% %depend on this kind of behaviour.
% %NS: behaviour is repeated so modified, pls check
% The magnetic turbulence further dictates the confinement of these charged particles in various astrophysical systems, ranging from jets to galaxies and clusters of galaxies.
% An analytical quasilinear model of diffusion \citep{jokipii_1966,jokipii_1973} has often been used to estimate diffusion coefficients when the turbulent field is relatively weaker than the background magnetic field.
% %Several studies, such as \citep{giacalone_1999,cesse_2001,candia_2004,fatuzzo_2010} have employed numerical simulations to examine the transport properties of charged particles in strong turbulence.
% For strong turbulence, on the other hand, several studies have employed numerical simulations to examine the transport properties of charged particles \citep{giacalone_1999,cesse_2001,candia_2004,fatuzzo_2010}.
% The majority of these research have focused their attention on the situation in which large-scale turbulence cascades toward smaller dissipative scales and the interaction between turbulent waves and charged particles is mediated by particular resonance conditions.
% Further in such studies, it is also implicitly assumed that the particles' gyro-radius is smaller than the maximum scale of the turbulence spectrum.

% However, under a number of physical circumstances, the particle's gyro-radius can surpass the maximum coherence length of the turbulence.
% For instance, the transport of supra-thermal particles in the vicinity of a relativistic shock, the propagation of very high-energy cosmic rays within a galaxy, the transport of particles through a medium of active magnetic reconnection, where the generation of small-scale turbulence is governed by the dissipation of magnetic energy, etc.
% Despite the wide application of this regime in several astrophysical systems, it has gained little attention to date.
% Although some recent research has been devoted to the study of this under-explored field, it has mostly focused on the problem of spatial transport.
% For example, \cite{plotnikov_2011} developed an analytical formulation of the spatial transport coefficients that is compatible with the numerical results for intense small-scale random magnetic field.
% Further, the work by \cite{subedi_2017} is worth noting which studies charged particle diffusion in entirely three-dimensional isotropic turbulent magnetic fields without a mean field. 

In this paper, we examine the momentum diffusive transport of charged particles in high-energy (or rigidity) regime with $R_{l}/l_{c}>>1$, where $R_{l}$ is the gyro-radius of the particle and $l_{c}$ is the highest correlation length of the turbulence.
Using an asymptotic analysis of the quasilinear diffusion coefficient, we estimate the transport coefficients corresponding to this regime.
We also demonstrate the impact of the interplay between stochastic Fermi acceleration due to small-scale turbulence and synchrotron loss on the spectrum of non-thermal particles.

The paper is organised in the following way: in section~\ref{sec:calc} we show the calculations for the momentum transport coefficient for small-scale turbulence and the results are shown in sections~\ref{sec:dpp} and \ref{sec:dmumu}. 
In section~\ref{sec:trans_dist}, we show the results from solving the cosmic ray Fokker-Planck equation using the calculated transport coefficient.
We discuss and summarize our findings in section~\ref{sec:diss} and in the appendix we lay-out all the required derivations.
%NS: looks OK, can be turned into plain text

==> results.tex <==
%\section{Results}\label{sec:res}
%\subsection{Transport coefficients}\label{sec:transport_coeff}
%\subsubsection{Momentum Diffusion $\left(D_{\gammaup \gammaup}\right)$}
%NS: modified section style, too much blank space otherwise

\section{Transport coefficients $D_{\gamma\gamma}$ and $D_{\mu\mu}$}
First, we present our results on the transport coefficients by numerically evaluating the integrals that appear in the expressions for $D_{\gamma\gamma}$ and $D_{\mu\mu}$ as presented above in section~\ref{sec:calc}. 
Subsequently, we solve the cosmic ray transport equation with the calculated diffusion coefficients in addition to the synchrotron loss process and study their interplay. 
\subsection{Momentum diffusion Coefficient $\left(D_{\gamma \gamma}\right)$}\label{sec:dpp}

\begin{figure}
    \centering
    \includegraphics[scale=0.44]{figures/Fig_1.png}
    \caption{Plot showing the dependence of $\xi=\frac{c}{P_{0}\Omega_{NR}^{2}}\displaystyle\int_{-1}^{1}D_{\gamma \gamma}\,\,d\mu$ on $\gamma$ for different values of $\beta_{A}$, $m'$ and $\sigma$. All the plots show the same trend of $\xi\propto\gamma^{-{2}/{3}}$, which is depicted by the black dashed line.}
    \label{fig:diff_gamm}
\end{figure}

\noindent
We are interested here in the average diffusion which is obtained by integrating $D_{\gamma\gamma}$ over the distribution of the pitch angle $\mu\in[-1,1]$.
Let us define such a dimensionless pitch-angle averaged momentum diffusion coefficient ($\xi$) as:
\begin{equation}
  \xi=\frac{c}{P_0\Omega_{NR}^{2}}\int_{-1}^{1}D_{\gamma\gamma}\,d\mu\,.
  \label{eq:xi}
\end{equation}
% This has dimensions of $[L]^{3}$.
In Fig.~\ref{fig:diff_gamm} we show the dependence of $\xi$ on $\gamma$ for different values of the parameters $\beta_{A}$, $m'$ and $\sigma$, which are all defined above in section~\ref{sec:calc}.
%, where $$\xi=\frac{c^{3}}{P_{0}\Omega_{NR}^{4}}\displaystyle\int_{-1}^{1}D_{\gammaup \gammaup}\,\,d\mu,$$
%is defined as the pitch-angle averaged $D_{\gammaup \gammaup}$ with dimension of $[L]^{3}$.
% The form is obtained by integrating Eq.~(\ref{eq:dpp}) over $x$ and $\mu$.
For all the plots shown in the figure, $\xi$ exhibits a power-law trend following the same exponent with the Lorentz factor $\gamma$ of the non-thermal particles, $\xi\propto\gamma^{-2/3}$. 
In the left panel, one can observe the increase in $\xi$ with increasing $\beta_{A}$ for a constant value of $m'=100\,\text{and}\,\sigma=5$.
This indicates that the higher the velocity of the Alfv\'{e}n wave is, {the quicker the non-thermal particles will diffuse in $\gamma$ space.}
% it will impart more energy to the particles. 
In the middle panel we show the dependence of $\xi$ on $\gamma$ for different values of $m'$.
{We observe} that with {increasing} $m'$, $\xi$ decreases for a fixed $\gamma$ value.
% However, this dependency changes for very high values of $m'$ ($>10^{8}$) where the power-law trend of $\xi$ deviates from its usual $\gamma^{-\frac{2}{3}}$ dependence and show a more steeper fall for higher $\gamma$ ($>10^{7}$) values.
Such behaviour of $\xi$ is expected as $m'$ parameterizes the scale of the turbulent energy injection, and higher values of $m'$ indicate that the energy is getting injected at a lower scale. 
The behaviour shown in the middle panel of the figure implies that such an energy injection at smaller scales reduces the momentum diffusion, resulting in the reduced acceleration of particles with large gyro-radii. 

In the right panel of the figure we show the functional dependence of $\xi$ on $\gamma$ for fixed $\beta_{A}$ and $m'$ but varying $\sigma$.
We observe with increasing $\sigma$ values the value of $\xi$ increases for a fixed $\gamma$ which is expected as with increasing $\sigma$, more and more Alfv\'{e}n waves would interact with the particles resulting in higher momentum diffusion $\xi$.

\subsection{Pitch-angle diffusion coefficient $\left(D_{\mu\mu}\right)$}\label{sec:dmumu}


\begin{figure}
    \centering
    \includegraphics[scale=0.44]{figures/Fig_2.png}
    \caption{Plot showing the dependence of $\chi=\frac{c}{P_{0}\Omega_{NR}^{2}}\displaystyle\int_{-1}^{1}D_{\mu \mu}\,\,d\mu$ on $\gamma$ for different values of $\beta_{A}$, $m'$ and $\sigma$. All the plots show the same trend of $\chi\propto\gamma^{-{8}/{3}}$, which is depicted by the black dashed line.}
    \label{fig:pitch_angle}
\end{figure}

\noindent
Similar to Eq.~(\ref{eq:xi}), we define another dimensionless pitch-angle averaged diffusion coefficient
$\chi$ as:
\begin{equation}
    \chi=\frac{c}{P_0\Omega_{NR}^{2}}\int_{-1}^{1}D_{\mu \mu}\,d\mu\,,
\end{equation}
with $D_{\mu \mu}$ being calculated by numerically integrating Eq.~(\ref{eq:dmumu}) for the region of $x$ satisfying Eq.~(\ref{eq:solutionx}).
In Fig.~\ref{fig:pitch_angle}, we plot $\chi$ for different values of $m'\,,\beta_{A}\, \text{and}\, \sigma$

All the plots exhibit an inverse power-law trend with Lorentz factor $\gamma$ of the cosmic rays.
For all the cases in the figure, we find the same power-law index of $-8/3$.
In the left panel of the figure, the plots are shown for constant $m'\,\text{and}\,\sigma$ but varying $\beta_{A}$.
The curves can be observed to almost overlap for different $\beta_{A}$, indicating that $\chi$ has a very weak dependency on the velocity of the Alfv\'{e}n waves.
%or on the value of the mean magnetic field in the turbulent medium.          
In the middle panel, the form of $\chi$ has been shown for different $m'$ values while $\beta_{A}\,\text{and}\,\sigma$ are kept constant.
Similar to $\xi$, here also we observe decrease in $\chi$ with increasing $m'$.
In the right panel of the figure we show the plots for different values of $\sigma$.
We find that $\chi$ increases with $\sigma$, which is expected as larger $\sigma$ consequently implies that more number of waves are interacting with the charged particles.
This results in more efficient diffusion.

\subsection{Solutions of the Fokker-Planck equation}\label{sec:trans_dist}
\begin{figure}
    \centering
    \includegraphics[scale=0.51]{figures/Fig_3.png}
    \caption{Evolution of an initial Gaussian (with mean $10^{4}$ and standard deviation $10^2$) for stochastic acceleration due to small-scale turbulence with different values of $D_{0}$ and following Eq.~(\ref{eq:acceleration}).
    The initial function is shown with a black dashed curve.}
    \label{fig:acceleration}
\end{figure}
\noindent
In this section we demonstrate the effect of the small-scale turbulence on the non-thermal particle spectrum by numerically solving the cosmic ray transport equation with the coefficients calculated in the earlier sections.
Note that all the numerical simulations are performed with a conservative, second order accurate IMEX scheme \citep{Kundu_2021} and considering a discretization of the the particle Lorentz factor $\gamma$ from $\gamma_{\min}=10^{3}$ to $\gamma_{\max}=10^{7}$ with $128$ logarithmically spaced bins to provide equal resolution per decade.

In a turbulent medium with a guided field, the transport of cosmic rays is governed by a Fokker-Planck equation of the following type \citep[][]{kirk_1988,schlickeiser_1998},
\begin{eqnarray}\label{eq:schlickeizer}
    \frac{\partial F}{\partial t} =\frac{\partial}{\partial z}\left(\mathcal{K}\frac{\partial F}{\partial z}\right)-\left(U+\frac{1}{4p^{2}}\left(\frac{\partial}{\partial p}p^{2}va_{1}\right)\right)\frac{\partial F}{\partial z} + \left(\frac{p}{3}\frac{\partial U}{\partial z}+\frac{v}{4}\frac{\partial a_{1}}{\partial z}\right)\frac{\partial F}{\partial p}+\frac{1}{p^{2}}\frac{\partial}{\partial p}\left(p^{2}a_{2}\frac{\partial F}{\partial p}\right)+S_{0}
\end{eqnarray}
% where $z$ is the spatial direction along the mean magnetic field, 
where $F$ is the pitch angle averaged cosmic ray distribution function, $U$ is the non-relativistic fluid velocity, $v$ is the velocity of the cosmic ray particle and $p$ is the momentum of the cosmic rays and  
\begin{eqnarray}\label{eq:kas}
    \mathcal{K}=\frac{v^{2}}{8}\int^{1}_{-1}d\mu\,\frac{(1-\mu^{2})^{2}}{D_{\mu\mu}},\quad a_{1}=\int_{-1}^{1}d\mu\,(1-\mu^{2})\frac{D_{\mu p}}{D_{\mu\mu}},\quad  a_{2}=\frac{1}{2}\int_{-1}^{1}d\mu\,\left(D_{pp}-\frac{D_{\mu p}^{2}}{D_{\mu\mu}}\right).
\end{eqnarray}
Note that while deriving Eq.~(\ref{eq:schlickeizer}) the background flow and the guided magnetic field are considered to be in the same spatial direction, $z$, and the timescale of pitch-angle scattering is assumed to be minimum among all the timescales present in the system. 
The latter assumption introduces the spatial diffusion term parallel to the guided magnetic field in the right hand side of the equation \citep{shalchi_2020}.
A term consisting diffusion of cosmic rays in the direction perpendicular to the guided field also arises in the Fokker-Planck equation due to the stochasticity in the magnetic field line structure \citep{shalchi_2021}.
For the current work such term due to perpendicular diffusion is neglected as quasilinear theory is unable to address such diffusive transport \citep{shalchi_2020}. 
As noted in the end of section~\ref{sec:calc}, $D_{\mu p}=0$ which gives $a_{1}=0$ and $a_{2}$ is simply the pitch-angle averaged $D_{pp}$.
For this work we consider averaging out the spatial coordinates and following the leaky-box approximation \citep{lerche_1985} we replace the spatial diffusion and convection term by a momentum dependent escape term \citep{rieger_2019} with an escape timescale defined as $T_{\rm esc}\sim\mathcal{K}^{-1}\propto \gamma^{-8/3}$.
Further considering the calculated forms for pitch-angle averaged diffusion coefficients (see section~\ref{sec:dmumu}) in addition to synchrotron cooling and neglecting adiabatic loss, Eq.~(\ref{eq:schlickeizer}) takes the following form (see appendix \ref{sec:transport} for a derivation),
\begin{eqnarray}\label{eq:transport}
    \frac{\partial f}{\partial T} +\frac{\partial}{\partial \gamma}\left(2a\gamma^{-\frac{5}{3}}-\gamma^{2}\right)f=\frac{\partial}{\partial \gamma}\left(a\gamma^{-\frac{2}{3}}\frac{\partial f}{\partial \gamma}\right)-b\gamma^{\frac{8}{3}}f
    + S,
\end{eqnarray}
where $a$, $b$ and $S$ are defined via Eq.~(\ref{eq:coeff_mod}).

Before considering the interplay of various micro-physical processes, we first analyze the effect of the acceleration due to small-scale turbulence only. 
For that, we numerically solve the following equation which is similar to Eq.~(\ref{eq:transport}) but without the synchrotron loss, particle escape, and injection,
\begin{eqnarray}\label{eq:acceleration}
    \frac{\partial f}{\partial T} +\frac{\partial}{\partial \gamma}\left(2D_{0}\gamma^{-\frac{5}{3}}\right)f=\frac{\partial}{\partial \gamma}\left(D_{0}\gamma^{-\frac{2}{3}}\frac{\partial f}{\partial \gamma}\right),
\end{eqnarray}
with $D_{0}$ being a parameter with which the efficiency of acceleration can be tuned.
% \sk{We numerically solve Eq.~(\ref{eq:acceleration}) to explore the effect of the stochastic acceleration due to small-scale turbulence on the non-thermal particle distribution.}

The numerical solution of Eq.~(\ref{eq:acceleration}) for different times and different $D_{0}$ values are shown in Fig.~\ref{fig:acceleration}.
Further the choice of the values for $D_{0}$ is motivated by considering the fitted form for $\xi$ with $\sigma=5$, $\beta=0.09$ and $m'=100$, $\xi\approx0.047\gamma^{-2/3}$, which results in a $D_{0}$ value of $\approx 10^{8}$ with a mean field of $10\,\mu$G.
An arbitrary Gaussian with $10^{4}$ and $10^{2}$ as mean and standard deviation respectively, has been considered as the initial distribution (shown by a black dashed curve). 
With time all the plots show the spreading of the initial distribution owing to the momentum diffusion and acceleration due to small-scale turbulence. 
However, the spreading of the initial distribution function is not uniform, the low energy part spreads faster than the high energy.
Such an acceleration can be analyzed by observing the dependency of the acceleration timescale, $\tau_{acc}$, on $\gamma$, which is $\tau_{acc}\sim \gamma^2/D\propto\gamma^{8/3}/D_{0}$ from Eq.~(\ref{eq:acceleration}).
It clearly shows that the timescale of acceleration is smaller for smaller $\gamma$, which explains the faster acceleration in the low energy part. 
The acceleration timescale also inversely depends on the choice of $D_{0}$, which is why we observe faster acceleration for higher values of $D_{0}$.

After analyzing various aspects and features of stochastic acceleration due to small-scale turbulence we now proceed to analyze the interplay of different micro-physical processes with this acceleration. 
To explore the combined effect of different processes on the distribution function, we numerically solve Eq.~(\ref{eq:transport}) with the above-mentioned algorithm by incorporating different processes gradually. 
% Further note that, for all the following simulations the $\gamma$ space is discretized from $\gamma_{\min}=10^{3}$ to $\gamma_{\max}=10^{7}$ with $128$ bins.


\begin{figure}
    \centering
    \includegraphics[scale=0.51]{figures/Fig_4.png}
    \caption{Evolution of an initial power-law energy distribution of the form $\gamma^{-6}$ following Eq.~(\ref{eq:transport}) considering synchrotron loss process and different values for $a$.
    The values for $b$ and $S$ are considered zero.
    The initial distribution is shown with the black dashed curve.}
    \label{fig:different_a}
\end{figure}

In Fig.~\ref{fig:different_a} we show the effect of the interplay of synchrotron loss process and particle acceleration due to small-scale turbulence on the particle distribution function.
We solve Eq.~(\ref{eq:transport}) with an initial power-law type particle distribution of the form,  $f(\gamma,0)\propto\gamma^{-6}$.
As has been shown in the previous section~\ref{sec:dpp}, the transport coefficients are dependent on the choice of the broadening $\sigma$ and injected power $P_{0}$,
which could be different for different astrophysical systems.
As an illustration, therefore, we solve Eq.~(\ref{eq:transport}) to demonstrate the
effects induced by the interplay of various micro-physical processes on the distribution function by varying $a$ and $b$ which are treated as arbitrary parameters in this work.
Nonetheless, we make some estimates for the parameter $a$ based on the same numbers
we chose earlier while estimating $D_{0}$ in the astrophysical settings. 
Noting that $a=D_{0} \gamma_s^{-11/3}/(c_0 B^2)$, we find $a\approx 10^{15}$, where $\gamma_{s}=10^3$ is chosen to scale the Lorentz factor $\gamma$ for computational purposes; see appendix \ref{sec:transport} for more details.


In the left panel of Fig.~\ref{fig:different_a} we show the evolution of the distribution function without the source and escape terms (considering $b=0$ and $S=0$ in Eq.~\ref{eq:transport}) and considering $a=10^{11}$.
The distribution function develops an exponential cut-off at higher $\gamma$, which moves towards lower energy as time progresses, due to synchrotron cooling.
Additionally a hump like structure can be observed to develop at the low energy regime due to the acceleration of low energy particles owing to the turbulent acceleration.
The overall distribution function attains a steady state as a result of the competition between stochastic acceleration and synchrotron loss. 
The form of the steady state distribution can be computed analytically from Eq.~(\ref{eq:transport}) considering $b=0$ and $S=0$ and is $\propto \gamma^{2}\,\exp\left\{-\Lambda(\gamma)\right\}$, where $\Lambda(\gamma)=3\left(\gamma^{{11}/{3}} - 1\right)/11a$ \citep[see Eq.~(A1) of][]{Kundu_2021}. 
Further, with such a steady state distribution function it can be observed that the maximum of the distribution occurs at $\left(2a\right)^{3/11}$ and it increases with $a$ which can be observed from the middle and the right panel of the figure where the evolution of the distribution is shown form $a=10^{13}$ and $a=10^{15}$ respectively. 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/Fig_5.png}
    \caption{Evolution of an initial power-law energy distribution of the form $\gamma^{-6}$ following Eq.~(\ref{eq:transport}) considering synchrotron loss process with different values for $a$ and $b=10^{-6}$.
    The values for $S$ is considered as zero.
    The initial distribution is shown with the black dashed curve.}
    \label{fig:1e-6_escape}
\end{figure}


In Fig.~\ref{fig:1e-6_escape}, we show the evolution of the distribution function including particle escape and acceleration along with synchrotron loss. The escape time is controlled by the parameter $b = 10^{-6}$ which is kept fixed for the curves shown with different $a$ values in three different panels. 
For all the plots the high-energy cut-off show a rapid decrement towards lower $\gamma$ as compared to Fig.~\ref{fig:different_a} owing to the particle escape in addition to the synchrotron loss process.
One interesting observation is that due to escape, the evolution of the distribution begins with the movement of the high-energy cut-off to lower $\gamma$ and increasing the rate of the evolution towards the steady state.
After attaining the steady state the movement of the cut-off towards lower $\gamma$ ceases and the height of the distribution starts to decrease as a result of the particle escape. 
Such kind of evolution is a manifestation of the escape time-scale which follows $\gamma^{-{8}/{3}}$ implying that the high-energy particles have lower escape time and therefore they leaks out of the system faster than the low energy particles. 
We further show the evolution of the distribution function for $b=10^{-4}$ and $10^{-5}$ with different $a$ values in Figs.~\ref{fig:1e-5_escape}, \ref{fig:1e-4_escape} which exhibit an almost similar evolutionary dynamics.
However, due to lesser escape timescale than with $b=10^{-6}$ the particles leaks out much faster for the cases presented in Figs.~\ref{fig:1e-5_escape}, \ref{fig:1e-4_escape}.

